The Milky Way Radial Metallicity Gradient as an Equilibrium Phenomenon: Why Old Stars are Metal-Rich

Metallicities of both gas and stars decline toward large radii in spiral galaxies, a trend known as the radial metallicity gradient. We quantify the evolution of the metallicity gradient in the Milky Way as traced by APOGEE red giants with age estimates from machine learning algorithms. Stars up to ages of $\sim$9 Gyr follow a similar relation between metallicity and Galactocentric radius. This constancy challenges current models of Galactic chemical evolution, which typically predict lower metallicities for older stellar populations. Our results favor an equilibrium scenario, in which the gas-phase gradient reaches a nearly constant normalization early in the disk lifetime. Using a fiducial choice of parameters, we demonstrate that one possible origin of this behavior is an outflow that more readily ejects gas from the interstellar medium with increasing Galactocentric radius. A direct effect of the outflow is that baryons do not remain in the interstellar medium for long, which causes the ratio of star formation to accretion, $\dot{\Sigma}_\star / \dot{\Sigma}_\text{in}$, to quickly become constant. This ratio is closely related to the local equilibrium metallicity, since its numerator and denominator set the rates of metal production by stars and hydrogen gained through accretion, respectively. Building in a merger event results in a perturbation that evolves back toward the equilibrium state on $\sim$Gyr timescales. Under the equilibrium scenario, the radial metallicity gradient is not a consequence of the inside-out growth of the disk but instead reflects a trend of declining $\dot{\Sigma}_\star / \dot{\Sigma}_\text{in}$ with increasing Galactocentric radius.

==> birth-radii.tex <==

\section{Birth Radius Inferences}
\label{sec:birth-radii}

\begin{figure}
\centering
\includegraphics[scale = 0.8]{lucys-calculations-fe.pdf}
\caption{
A comparison between our models and the methodology presented by \citet{Lu2022b} for estimating birth radii for stars (see discussion in section \ref{sec:discussion:birth-radii}).
Range(\onh{Fe}) refers to the difference between the 5th and 95th percentiles of the MDF, shown here in 1-Gyr bins of age for stars between $R = 7$ and $10$ kpc.
Stars mark \citepossessivepar{Lu2022b} measurements using data from LAMOST (blue) and the same measurements for our sample from APOGEE (red).
Lines, color coded and styled according to the legend, mark the predictions by our \modelname{Exp}{2} model and variations thereof (see discussion in sections \ref{sec:gce:primary-set} and \ref{sec:gce:variations}).
{\bf Summary}: The relationship between Range(\onh{Fe}) and is influenced to some extent by stellar migration.
Modeling these effects would improve the \citet{Lu2022b} methodology.
}
\label{fig:lu-comparison}
\end{figure}

In section \ref{sec:discussion:birth-radii}, we discussed the recent method put forth by \citet{Lu2022b} for determining Galactocentric birth radii based on the relationship between the width of the \onh{Fe} distribution and stellar population age.
Therein we raised concerns about the reliability of this methodology.
We discuss this point further in this appendix.
\par
To compare the arguments by \citet{Lu2022b} with our models, we apply their methodology to our predictions.
To mimic measurement uncertainty, we perturb the ages and metallicities of each stellar population by random numbers drawn from normal distributions of width $0.5$ Gyr and $0.03$ dex, respectively.
We then isolate stellar populations between $R = 7$ and $10$ kpc at the present day and take Range(\onh{Fe}) to be the difference between the 5th and 94th percentiles of the \onh{Fe} distribution for a mono-age population.
We apply the same procedure to our sample from APOGEE but omit the perturbation by artificial uncertainties.
\par
Fig. \ref{fig:lu-comparison} shows the results of this procedure as a function of stellar population age in comparison to the LAMOST subgiants from \citet{Lu2022b}.
The APOGEE stars follow a similar trend as LAMOST.
The two surveys are in good agreement with one another, considering systematic uncertainties that can arise when comparing optical and infrared surveys with different radial coverage of the disk.
\citet{Ratcliffe2023} also used APOGEE stars, but with ages measured with {\sc XGBoost} \citep{Miglio2021}, a supervised machine learning algorithm based on spectroscopically inferred stellar parameters and asteroseismic ages.
Our measurements are in reasonable qualitative agreement with theirs, but with some differences in detail (see their Fig. 2).
\par
We show Range(\onh{Fe}) as a function of age predicted by our \modelname{Exp}{2} and \modelname{Exp}{2}+burst models along with the variations that use 25\% faster and slower radial migration from section \ref{sec:discussion:migration}.
Our models predict systematically narrower MDFs than observed.
This discrepancy does not affect our main conclusions, because the arguments in this paper are based on the position of the mode of the distribution as opposed to its detailed shape.
One potential origin of this discrepancy is short timescale (of order $\sim$$100$ Myr) variations in the ISM metallicity, which should in principle arise due to the clumpy and episodic nature of accretion and star formation.
Such effects are not present in our GCE models in this paper, because we use smooth SFHs.
\par
Despite a nearly constant slope $\grad{Fe}$, the \modelname{Exp}{2} model and its variations each predict Range(\onh{Fe}) to increase by $\sim$$0.2$ dex between young and $\sim$$10$ Gyr old populations.
This prediction is a consequence of radial migration.
The $R = 7 - 10$ kpc range, which this comparison focuses on, samples a broader range of birth radii with increasing age.
Due to the presence of a radial abundance gradient, this region therefore also samples a broader range of metallicities.
The trend depends minimally on the strength of radial mixing, but there is a trend nonetheless.
As mentioned in section \ref{sec:discussion:birth-radii}, we therefore raise concerns regarding the reliability of birth radii determined with this method.
A portion of this trend should be attributed to radial migration, and therefore variations in Range(\onh{Fe}) and $\grad{Fe}$ with age should have different shapes.
\par
We nonetheless support the argument by \citet{Lu2022b} that Range(\onh{Fe}) should increase and $\grad{Fe}$ should decrease briefly during a merger event.
Our \modelname{Exp}{2}+burst model predicts Range(\onh{Fe}) to increase by $\sim$$0.1 - 0.2$ dex at a time coincident with the enhanced accretion associated with this model.
It is therefore reasonable to infer that the GSE merger event \citesomeone\ would have simultaneously steepened the Galactic abundance gradient and increased MDF widths $\sim$$8 - 12$ Gyr ago.
These effects are not apparent in our measurements with APOGEE, but that discrepancy could be an issue of systematic differences between the surveys.



% {\color{red} Copied over from the old version of section \ref{sec:discussion:birth-radii}. Needs editing.}
% \par
% To compare results, we apply their methodology as described in their Appendix A to our \modelname{Exp}{3}, \modelname{evolExp}{3}, and \modelname{Exp}{3}+burst models (see discussion in section \ref{sec:gce:variations}).
% To mimic measurement uncertainty, we perturb the predicted ages and metallicities of each stellar populations by 0.5 Gyr and 0.03 dex, respectively.
% We then isolate stellar populations between $R = 7$ and $10$ kpc at the present day and take Range(\onh{Fe}) to be the difference between the 5th and 95th percentiles of the \onh{Fe} distribution for a mono-age population.
% We apply the same procedure to our sample from APOGEE.
% \par
% Fig. \ref{fig:lu-comparison} shows the results of this procedure as a function of stellar population age in comparison to \citepossessivepar{Lu2022b} measurements with LAMOST subgiants.
% The APOGEE stars follow a similar trend as LAMOST but with significantly lower normalization, indicating that the width of the MDF is systematically different between the two surveys.
% It is likely that this difference in Range(\onh{Fe}) accounts for a portion of the difference in metallicity gradient slopes that we infer.
% We found a value of $\grad{Fe} = -0.07$ kpc$^{-1}$ (see Table \ref{tab:regressions} and Fig. \ref{fig:gradients}), whereas \citet{Lu2022b} found values closer to $\grad{Fe} = -0.1$ kpc$^{-1}$ depending on stellar population age.
% \citet{Ratcliffe2023} recently applied the \citet{Lu2022b} methodology to APOGEE stars with ages from {\sc XGBoost} \citep{Miglio2021}, a supervised machine learning technique based on spectroscopically inferred stellar parameters and asteroseismic ages.
% They found an even lower normalization to this trend, with values of Range(\onh{Fe}) $\approx 0.2$ for $\sim$$3 - 5$ Gyr old stars.
% \par
% Our GCE models qualitatively reproduce the trend, but with a lower normalization than both \citepossessivepar{Lu2022b} LAMOST sample and our APOGEE sample.
% The distribution widths that we predict are in reasonable agreement with \citepossessivepar{Ratcliffe2023} measurements (see their Fig. 2).
% Most importantly, our \modelname{Exp}{3}+burst model exhibits an increase in Range(\onh{Fe}) at an age that is coincident with the burst of star formation built into this model.
% The enhanced accretion in the outer disk that fuels the burst also steepens the metallicity gradient at this time (see Fig. \ref{fig:outerburst}).
% We therefore support the argument by \citet{Lu2022b} that major merger events should simultaneously steepen the ISM metallicity gradient and widen the \onh{Fe} distribution of mono-age populations.
% \par
% However, our \modelname{Exp}{3} and \modelname{evolExp}{3} models also predict trends in Range(\onh{Fe}) with age.
% In particular, the \modelname{Exp}{3} model reasonably matches the measurement by \citet{Ratcliffe2023}.
% This model, by construction, predicts an ISM metallicity gradient that does not evolve significantly over the last $\sim$$10$ Gyr of thin disk evolution.
% In the \modelname{evolExp}{3} model, the slope evolves significantly only in the $\tau \approx 3.5 - 5$ Gyr range of lookback times (see Fig. \ref{fig:eta-sudden-change}).
% \par
% We therefore raise concerns regarding the reliability of birth radii inferred with this method, as in \citet{Lu2022b} and \citet{Ratcliffe2023}.
% In our GCE models, these trends arise as a consequence of stellar migration.
% With increasing age, stars in the solar annulus sample a wider and wider range of birth radii, and by extension a wider and wider range of metallicities (see also Fig. 15 of \citealt{Johnson2021}).
% The ISM metallicity gradient therefore need not evolve in order for this trend to arise if stars are allowed to migrate radially.
% A more precise understanding of the dynamical mixing history of the MW is required in order to model its effects and more reliably use the information on birth radii encoded in the dispersion of metallicities in mono-age populations.

